Calibrated Predictive Safety for Heterogeneous Robots: An Action-Conditioned JEPA Framework with Model-Based Safety Shields

Vision-language-action policies generalize broadly but provide no execution-time guarantees; classical model-based planners respect kinematic and geometric constraints but generalize poorly. We study whether an action-conditioned Joint-Embedding Predictive Architecture (JEPA) world model can predict, before execution, both task progress and physical risk for candidate action chunks, and whether coupling these predictions to an embodiment-specific model-based safety shield yields a deployable pipeline for heterogeneous robots. We propose a receding-horizon decision pipeline: (1) a proposer produces K candidate action chunks; (2) an action-conditioned JEPA rolls each candidate forward in a frozen-encoder latent space conditioned on an embodiment embedding; (3) calibrated risk and progress heads score each rollout and report uncertainty; (4) a deterministic per-embodiment safety shield filters inadmissible candidates; (5) a fallback ladder handles empty-admissible-set cases. The learned ranking only reorders admissible candidates; enforcement guarantees come from the deterministic shield and fallback ladder. We evaluate with a pre-registered protocol in simulation (LIBERO-Long). In 600-episode configurations the full framework improved success over a shield-only baseline and reduced collision false negatives at matched recall. Deployment-efficiency measurements on target on-robot and edge accelerators are included. Real-robot experiments and an offline reranking significance test remain future work; see the paper for disclosures.

==> sections/disclosure.tex <==
\section*{Scope and honesty statement}
\label{sec:disclosure}

This manuscript is a systems, framework and evaluation-protocol paper
with a partial first-party empirical execution. Concretely: (i) every
number attributed to prior work is quoted from that work and cited to
a specific table or section (\texttt{source\_notes.md}); (ii) Level~2
(predictive/calibration) and Level~4 (closed-loop) of the protocol in
Sec.~\ref{sec:levels} have been executed on the LIBERO-Long simulator
and are reported as measurements, not placeholders, in
Tables~\ref{tab:prediction} and~\ref{tab:closedloop};
(iii) Figs.~\ref{fig:calibration}--\ref{fig:rocpr} are computed from
real per-example Level-2 predictions, but Level~3 (offline reranking
significance) has not been executed, and we do not show a
candidate-score figure built from synthetic data in its place
(Sec.~\ref{sec:candidatefig}); (iv) no result in this paper
comes from a physical robot
or from more than one embodiment; (v) we
make no claim of priority, no claim that a single control policy
transfers unmodified across embodiments, and no claim of formal safety
guarantees from the learned components --- every guarantee originates
from the shield (Sec.~\ref{sec:shield}) and the fallback ladder
(Sec.~\ref{sec:fallback}). Sec.~\ref{sec:todo} lists exactly what
remains before the outstanding empirical claims may be asserted.

